Steady-states of thin film droplets on chemically heterogeneous substrates

We study steady-state thin films on a chemically heterogeneous substrates of finite size, subject to no-flux boundary conditions. Based on the structure of the bifurcation diagram, we classify the one-dimensional steady-state solutions that exist on such substrates into six different branches and develop asymptotic estimates for the steady-states on each branch. We show using perturbation expansions, that leading order solutions provide good predictions of the steady-state thin films on stepwise-patterned substrates. The analysis in one dimension can be extended to axisymmetric solutions. We also examine the influence of the wettability contrast on linear stability and dynamics. Results are also applied to describe two-dimensional droplets on hydrophilic square patches and striped regions used in microfluidic applications.

==> bob_macros.tex <==
%----  macros to save typing; added by hartley, 2002 ----
\newcommand{\fig}{\begin{figure}[htbp]\centering}
\newcommand{\pic}[1]{\includegraphics[width=#1]}
\newcommand{\efig}{\end{figure}} 
%\newcommand{\efig}{\end{figure} \clearpage}
% Use \clearpage to cure ``too many floats'' problem (1 fig. per page).
\newcommand{\fr}[1]{Figure \ref{fig:#1}}
\newcommand{\FR}[1]{Figure \ref{fig:#1}}
\newcommand{\er}[1]{equation \ref{eq:#1}}
\newcommand{\ER}[1]{Equation \ref{eq:#1}}
\newcommand{\eq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\eqa}{\begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray}}
\newcommand{\etal}{\nobreak\mbox{\it et al.}}



\newcommand{\singlespacing}{%
  \let\CS=\small\renewcommand{\baselinestretch}{1.0}\CS}
\newcommand{\doublespacing}{%
  \let\CS=\small\renewcommand{\baselinestretch}{1.6}\CS}
\newcommand{\normalspacing}{\doublespacing}

%\newcommand{\singlespacingplus}{%
%  \let\CS=\@currsize\renewcommand{\baselinestretch}{1.25}\tiny\CS}
%\newcommand{\realdoublespacing}{%
%  \let\CS=\@currsize\renewcommand{\baselinestretch}{2}\tiny\CS}
%\newcommand{\footnotespacing}{\singlespacing}
%\newcommand{\changespacing}[2]{%
%  \renewcommand{#1}{%
%    \let\CS=\@currsize\renewcommand{\baselinestretch}{#2}\tiny\CS}%
%}
%\newcommand{\changenormalspacing}[1]{\renewcommand{\normalspacing}{#1}}




%---- units ----
\newcommand{\days}{\nobreak\mbox{$\;$days}}
\newcommand{\hrs}{\nobreak\mbox{$\;$hrs}}
\newcommand{\mins}{\nobreak\mbox{$\;$min}}
\newcommand{\s}{\nobreak\mbox{$\;$s}}
\newcommand{\ms}{\nobreak\mbox{$\;$ms}}
\newcommand{\us}{\nobreak\mbox{$\;\mu$s}}
\newcommand{\inch}{\nobreak\mbox{$\;$in}}
\newcommand{\meter}{\nobreak\mbox{$\;$m}}
\newcommand{\cm}{\nobreak\mbox{$\;$cm}}
\newcommand{\mm}{\nobreak\mbox{$\;$mm}}
\newcommand{\um}{\nobreak\mbox{$\;\mu$m}}
\newcommand{\nm}{\nobreak\mbox{$\;$nm}}
\newcommand{\cmpers}{\nobreak\mbox{$\;$cm\,s$^{-1}$}}
\newcommand{\mmpers}{\nobreak\mbox{$\;$mm\,s$^{-1}$}}
\newcommand{\umpers}{\nobreak\mbox{$\;\mu$m\,s$^{-1}$}}
\newcommand{\g}{\nobreak\mbox{$\;$g}}
\newcommand{\kg}{\nobreak\mbox{$\;$kg}}
\newcommand{\hz}{\nobreak\mbox{$\;$Hz}}
\newcommand{\mhz}{\nobreak\mbox{$\;$mHz}}
\newcommand{\uhz}{\nobreak\mbox{$\;\mu$Hz}}


%---- oft-used complicated symbols ----
\newcommand{\rms}{\nobreak\mbox{$\sigma_{rms}$}}
\newcommand{\sat}{\nobreak\mbox{$\sigma_{\textrm{sat}}$}}
\newcommand{\DG}{\nobreak\mbox{$\Delta G^2$}}
\newcommand{\DS}{\nobreak\mbox{$\Delta\sigma$}}
\newcommand{\DQ}{\nobreak\mbox{$\Delta\theta$}}
\newcommand{\DSDQ}{\nobreak\mbox{$\Delta\sigma/\Delta\theta$}}
\newcommand{\dq}{\nobreak\mbox{$d\theta$}}
\newcommand{\ds}{\nobreak\mbox{$d\sigma$}}
\newcommand{\dsdq}{\nobreak\mbox{$d\sigma/d\theta$}}
\newcommand{\YY}{$\curlyvee\curlywedge$}
\newcommand{\GG}{\nobreak\mbox{$G^2$}}



==> imamat_class file_2012/bob_macros.tex <==
%----  macros to save typing; added by hartley, 2002 ----
\newcommand{\fig}{\begin{figure}[htbp]\centering}
\newcommand{\pic}[1]{\includegraphics[width=#1]}
\newcommand{\efig}{\end{figure}} 
%\newcommand{\efig}{\end{figure} \clearpage}
% Use \clearpage to cure ``too many floats'' problem (1 fig. per page).
\newcommand{\fr}[1]{Figure \ref{fig:#1}}
\newcommand{\FR}[1]{Figure \ref{fig:#1}}
\newcommand{\er}[1]{equation \ref{eq:#1}}
\newcommand{\ER}[1]{Equation \ref{eq:#1}}
\newcommand{\eq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\eqa}{\begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray}}
\newcommand{\etal}{\nobreak\mbox{\it et al.}}



\newcommand{\singlespacing}{%
  \let\CS=\small\renewcommand{\baselinestretch}{1.0}\CS}
\newcommand{\doublespacing}{%
  \let\CS=\small\renewcommand{\baselinestretch}{1.6}\CS}
\newcommand{\normalspacing}{\doublespacing}

%\newcommand{\singlespacingplus}{%
%  \let\CS=\@currsize\renewcommand{\baselinestretch}{1.25}\tiny\CS}
%\newcommand{\realdoublespacing}{%
%  \let\CS=\@currsize\renewcommand{\baselinestretch}{2}\tiny\CS}
%\newcommand{\footnotespacing}{\singlespacing}
%\newcommand{\changespacing}[2]{%
%  \renewcommand{#1}{%
%    \let\CS=\@currsize\renewcommand{\baselinestretch}{#2}\tiny\CS}%
%}
%\newcommand{\changenormalspacing}[1]{\renewcommand{\normalspacing}{#1}}




%---- units ----
\newcommand{\days}{\nobreak\mbox{$\;$days}}
\newcommand{\hrs}{\nobreak\mbox{$\;$hrs}}
\newcommand{\mins}{\nobreak\mbox{$\;$min}}
\newcommand{\s}{\nobreak\mbox{$\;$s}}
\newcommand{\ms}{\nobreak\mbox{$\;$ms}}
\newcommand{\us}{\nobreak\mbox{$\;\mu$s}}
\newcommand{\inch}{\nobreak\mbox{$\;$in}}
\newcommand{\meter}{\nobreak\mbox{$\;$m}}
\newcommand{\cm}{\nobreak\mbox{$\;$cm}}
\newcommand{\mm}{\nobreak\mbox{$\;$mm}}
\newcommand{\um}{\nobreak\mbox{$\;\mu$m}}
\newcommand{\nm}{\nobreak\mbox{$\;$nm}}
\newcommand{\cmpers}{\nobreak\mbox{$\;$cm\,s$^{-1}$}}
\newcommand{\mmpers}{\nobreak\mbox{$\;$mm\,s$^{-1}$}}
\newcommand{\umpers}{\nobreak\mbox{$\;\mu$m\,s$^{-1}$}}
\newcommand{\g}{\nobreak\mbox{$\;$g}}
\newcommand{\kg}{\nobreak\mbox{$\;$kg}}
\newcommand{\hz}{\nobreak\mbox{$\;$Hz}}
\newcommand{\mhz}{\nobreak\mbox{$\;$mHz}}
\newcommand{\uhz}{\nobreak\mbox{$\;\mu$Hz}}


%---- oft-used complicated symbols ----
\newcommand{\rms}{\nobreak\mbox{$\sigma_{rms}$}}
\newcommand{\sat}{\nobreak\mbox{$\sigma_{\textrm{sat}}$}}
\newcommand{\DG}{\nobreak\mbox{$\Delta G^2$}}
\newcommand{\DS}{\nobreak\mbox{$\Delta\sigma$}}
\newcommand{\DQ}{\nobreak\mbox{$\Delta\theta$}}
\newcommand{\DSDQ}{\nobreak\mbox{$\Delta\sigma/\Delta\theta$}}
\newcommand{\dq}{\nobreak\mbox{$d\theta$}}
\newcommand{\ds}{\nobreak\mbox{$d\sigma$}}
\newcommand{\dsdq}{\nobreak\mbox{$d\sigma/d\theta$}}
\newcommand{\YY}{$\curlyvee\curlywedge$}
\newcommand{\GG}{\nobreak\mbox{$G^2$}}



==> imamat_class file_2012/intro.tex <==
% The \vspace{} command in this chapter is just for aesthetic reasons - I don't like something new to start at the last line 
%of the page

% ONE OF THE BEST ONLINE LATEX REFERENCES IS AT :
% http://www.eng.cam.ac.uk/help/tpl/textprocessing/latex_advanced/latex_advanced.html

%% ALL figures are in EPS format: It is the best possible format 

\vspace{0.2in}

Thin liquid films on solid substrates are often seen in nature and technology, for example, as tear film on the eye, lubricating coating and functional layers in microfluidic devices \cite{thiele2003modelling}. Microfluidics refers to systems that manipulate small amounts of fluids, using channels with dimensions at scale of micrometer \cite{whitesides2006origins}. Microfluidics has found many applications in cell biology and chemical synthesis \cite{whitesides2006origins,lo2013application}. In biology, microfluidic system is used to manipulate cells, such as separation of motile and nonmotile cells, observing and growing cells. Compared to conventional tissue culture dish, analysis of stem cells can be done in a much more systematic way using microfluidics devices \cite{zhang2012applications}. The development of practical microanalytical systems has also advanced the technology in the analysis of biological samples such as blood, faeces and soil \cite{whitesides2006origins}. Lo mentions that in chemistry, microfluidic devices have been recently used as a powerful tool for process intensification because of their low fabrication costs, safe operation, and capability of integrating multiple basic steps onto one chip \cite{lo2013application}. \smallskip

Typically, films are considered as thin if their thickness is much smaller than their length. Due to the small aspect ratio of thin films, the Navier-Stokes equation describing the motion of an incompressible Newtonian liquid film can be approximated by a nonlinear partial differential equation (PDE) after nondimensionalization. The simplified PDE which is also known as lubrication approximation describes the evolution of thin film thickness. To understand the dynamics of thin film evolution, lubrication approximation has been used to study many physics problems involving the flow of thin films. This chapter briefly reviews the literature of lubrication approximation applied to different physics contexts and concludes with the plan of the dissertation.

\section{Thin film on homogeneous substrates}

Depending on the driving force of the thin film, the dominant effects in the lubrication approximation are different. If the driving force is gravity, then the viscous forces and gravity term are of the same order. If the driving force is surface tension, then the viscous force and surface tension balance. Along with the driving force, the intermolecular interaction between the fluid film and solid substrate also plays a critical role in determining the thickness profile of the thin film. Under the influence of van der Waals attractive forces and short-range repulsive forces, droplets may form. The interaction between the film and the solid substrate is modeled by a disjoining pressure function. The pressure in the thin film is determined by both the driving force and the intermolecular force. The shape of a liquid droplet is determined by the combination of surface tension and external forces. The contact angle of a droplet quantifies the wetting property of a solid surface. The study on wettability of solid substrates is particularly useful for applications such as oil recovery, liquid coating and inkjet printing \cite{zhao2010pore,sakai2008effect,bhushan2009lotus,dong2006visualization,son2008spreading,yuan2013contact}. Specifically, the design of superhydrophobic surfaces have attracted many recent research interests due to its applications in self-cleaning windows and systems that require minimizing drag in fluid flow \cite{bhushan2009lotus,yuan2013contact}.
\smallskip

We know that droplets are spherical in shape so that the surface area exposed is minimized given a fixed volume. However, classical solutions given by spherical shapes are inadequate capturing the thin film profiles in all physics phenomena \cite{mac2016new}. More quantitative analysis is needed to improve the accuracy of the thin film models. The understanding of the thin film at equilibrium is particularly important for capturing features of thin films such as contact angle, pressure, and position of the droplets \cite{mac2016new}. The steady-state profile of thin film droplets has been studied by numerical methods, asymptotic approximations and ellipsoidal droplet modeling \cite{mac2016new,gomba2009analytical, glasner03coarsening,lubarda2011analysis}. The different forms of disjoining pressure considered directly affects the complexity of the steady-state calculations. Different regimes have been identified and used in approximating steady-states under the influence of different wetting properties of the thin film \cite{gomba2009analytical,glasner03coarsening,bertozzi2001dewetting}. Glasner and Witelski consider the steady-state thin film parameterized by pressure on an infinite domain, specifically the homoclinic solution. They derive an parabolic approximation for large droplets using asymptotic matching \cite{glasner03coarsening}. Bertozzi, Grun and Witelski present a similar analysis and calculation for steady-states for thin film on a finite domain. Instead of focusing on the homoclinic solution, they study the periodic steady-states with a fixed domain size, including their asymptotic solution, bifurcation structure and stability \cite{bertozzi2001dewetting}. 
\smallskip

The presence of intermolecular interaction between the film and solid substrate can cause instabilities in thin film that lead to the formation of droplets on thin films. This process is also known as dewetting. In the late stages of dewetting, droplets evolve slowly by means of translation and mass change \cite{glasner2005collision}. The increase or decrease in the total number of droplets as a result of droplet movement and mass change is known as coarsening. One technique to study the coarsening dynamics is through Coarsening Dynamical System (CDS) \cite{watson2003coarsening}. The characterization of coarsening process using CDS allows an understanding of both the associated scaling laws and statistical information about the coarsening behavior \cite{chapman2012coarsening}. By introducing a slow time scale and employing solvability conditions given by Fredholm Alternative, Glasner and Witelski have derived a finite dimensional system of ODEs from the full evolution equation in 1-D. The reduced ODE system obtained is similar to that derived for Cahn-Hilliard equation, which is also a set of ODEs describing the evolution of the position of the kinks \cite{argentina2005coarsening,bates1994metastable}. Glasner and Witelski have demonstrated that the approximated ODE system gives a good prediction of position and pressure for large droplets in presence of small fluxes at the boundary\cite{glasner03coarsening}.
\smallskip

\section{Thin film on heterogeneous substrates}

Much theoretical understanding of thin films has been limited to film on homogeneous substrates. However, most of the naturally occurring surfaces are chemically heterogeneous due to contamination, cavities, etc. Tailored chemically heterogenous substrates are also increasingly used for the engineering of micropatterns of thin films \cite{zope2001self}. 
%[Check Refs 35-43] 
\smallskip

Liquid flow on chemically patterned substrate has been studied extensively due to its various applications in microfluidics. One application is in the design of the chemical patterns of the nozzle plate in inkjet print heads \cite{kooij2012directional}. Inkjet technology makes use of tiny ink drops to recreate digital image. Due to its non-contacting nature, it can be used to print on various media. It is also widely used to print electronics. Thin film transistors, inverters and active-matrix backplanes have been fabricated by inkjet printing technique \cite{kawase2003inkjet}. Quantifying the characteristics of wetting layer on the nozzle plate is critical to improving the printing quality and resolution \cite{kooij2012directional}. Another application can be found in microcontact printing where a stamp is used to transfer the material onto a substrate to create a desired pattern. The pattern is generated through contact between the stamp and the surface \cite{darhuber2000morphology}. Understanding the shape of liquids at equilibrium on chemically patterned substrate is essential to optimizing the printing process \cite{darhuber2000morphology}.
\smallskip



Kargupta et al. study the instability and pattern formation in thin film on chemically heterogeneous substrates with a stepwise pattern. On such a substrate, they identify a mode of surface instability caused by the spatial gradient of intermolecular force across the solid substrate. By performing a linear stability analysis of the thin film equation, they compute the characteristic time scale for the growth of instability and verify that the time scale is inversely proportional to the potential difference caused by heterogeneity.  They show that the introduction of heterogeneity can destabilize spinodally stable films and reduce the time of rupture for thicker films \cite{kargupta2002morphological,kargupta2000instability}. Lenz and Lipowsky investigate the morphologies of different equilibrium states of liquids on a surface that consists of hydrophilic domains in a hydrophobic matrix. By minimizing the interfacial free energy subject to the constant liquid volume, they find that the different morphologies are determined by the liquid volume and the area fraction of the hydrophilic domains. They also identify the transition among three different regimes using liquid volume as a parameter \cite{lenz1998morphological}. On a chemically heterogeneous substrate, the contact angle may no longer be described by Young's equation. Kooij et al. show that on a stripe-patterned surface, the contact angle formed can be well approximated using Cassie's law in terms of the width ratio of the two different stripes \cite{kooij2012directional}. Kaspar et al. explore the effect of alternating hydrophobic and hydrophilic area on a rectangular micro-arrayed surface on the confinement and spillover of water droplets on flat surfaces. They derive the contact angle as an arctan function of drop height using the spherical cap geometry with a coefficient that accounts for the properties of the confining surface \cite{kavspar2016confinement}.  \smallskip

Thiele has studied the effect of a smoothly patterned substrate on stationary droplet profile using wettability as a control parameter \cite{thiele2003modelling}. Their work considers heterogeneous substrate modeled by a sinusoidal modulation with a small amplitude. By varying the amplitude and periodicity of the chemical pattern, they identify the parameter range where the pinning mechanism emerges from coarsening. Kao, Golovin and Davis have also studied the effect of small wettability contrast with sinusoidal modulation on the steady-state thin film profile with and without rupture \cite{kao2006rupture}. In addition, stepwise patterned substrate with small wettability contrast has also been studied. Imperfect bifurcation has been observed in bifurcation diagram for films on heterogeneous substrate \cite{kao2006rupture}. By using weakly nonlinear analysis, they derive predictions for steady-state droplet shape, stability and rupture time on square-wave patterned substrate. By using both experiments and numerical simulations, Brasjen and Kondic study dewetting on chemically patterned heterogeneous substrate with a focus on the dynamics of fluid fronts \cite{brasjen2013dewetting,kondic2004instabilities}.
\smallskip

\section{Plan of the dissertation}
This dissertation focuses on the mathematical models of dynamics and steady-states of thin liquid film on chemically homogeneous and heterogeneous substrates. The plan of this dissertation is shown as follows.
\begin{itemize}
\item In Chapter 2, we show the derivation of lubrication equation which describes the flow of thin liquid film of viscous fluid from Navier-Stokes equation. In particular, we consider the lubrication equation with both attractive and repulsive van der Waals potential, driven by surface tension.
\item In Chapter 3, we present results on the droplet-type steady-state solutions on homogeneous substrate. We show that the steady-state homoclinic droplet in the limit of small mass can be approximated by a hyperbolic trigonometric function to leading order. We also examine and discuss the stability of periodic steady-state solutions through a linear stability analysis approach.
\item In Chapter 4, we first examine the simplified model proposed by Glasner and Witelski and demonstrate the limitation of the model as the magnitude of the flux increases. Then we present the derivation and numerical simulations of an improved model predicting the single-droplet behavior on a finite domain by modifying the asymptotic expansion used previously by Glasner and Witelski.
\item In Chapter 5, we study the 1-D steady-state solutions of thin films on chemically heterogeneous substrates. We consider the thin film flow on a substrate of finite length and piece-wise patterned material property. We examine the structure of the bifurcation diagram by classifying the bifurcation diagram into six different branches. We derive the asymptotic prediction of the steady-state solutions that exist on each branch and extend the results to axisymmetric solution on 2-D domains.
\item In Chapter 6, we discuss future directions of dewetting and steady-state thin liquid films, including a refined model predicting the dynamics of thin film evolution that extends to multiple droplets in the same domain, the dynamics of thin films on 2-D homogeneous and heterogeneous substrates, and the steady-state thin film on 2-D heterogeneous substrates in the limit of small and large heterogeneity contrast. 
\item Appendix A provides the details of the numerical methods used in the numerical simulations of the PDE.

\end{itemize}



%Kaj neoficialaj kunvenas sur neuxtrala tereno. Kernan eron en kursoj por. Almenaux unu fremdan lingvon gxis parola grado Multokaze tio kondukas! Gxi ne estas bazita sur respekto, kaj malgrandaj devus disponi pri reala sxanco! Lingvoj estas recepto por konstanta. Oni ankaux rekomendas Esperanton kiel kernan. Lingvo kiel cxiu vivajxospecio estas valora jam pro si mem kaj inda je, firmaj radikoj cxe sia loka kultura kaj lingva identeco! Por multaj lernantoj kiuj tamen profitus el la scio de dua lingvo. 
%
%\vspace{0.2in} 
%
%% A simple way to make sections
%\section{Section}
%Lingva diverseco Homa emancipigxo Cxiu lingvo liberigas, kaj lingva identeco sed ne limigite de ili Ni asertas ke la ekskluziva!\cite{nawahi1928} La grandan diversecon de lingvoj en la mondo kiel baron. Profitus el la scio de dua lingvo Ni estas movado por efika. Etna lingvo estas ligita al difinita perspektivo pri la. 
%
%Gxi ne estas bazita sur respekto al kaj subteno de cxiuj. Propedeuxtikajn efikojn al la lernado de aliaj lingvoj Oni ankaux rekomendas Esperanton kiel kernan eron.
%
%
%\vspace{0.2in}
%
%% An example of making lists of various kinds - This one gives black circles of certain size based on style files - 
%% LaTeX manual will tell you how to put numbers or different symobols
%
%
%Naciaj lingvoj neeviteble  En la Esperantokomunumo la anoj. Al cxiu homo partopreni kiel.  La, sed ne limigite de ili . 
%
%Definitions used here:\begin{itemize}
%\item \emph{Naciaj} lingvoj neeviteble starigas barojn al.
%\item \emph{Starigas} barojn al, cxe granda parto de la monda logxantaro.
%\item \emph{La lingvo} Ni estas movado por lingvaj rajtoj Lingva diverseco.
%\item Ni asertas ke la ekskluziva uzado de naciaj lingvoj \emph{hoarder}.
% \end{itemize}
%
%% Ah! a little bit of math - all math is between two "$" signs
%
%Starigas barojn al, cxe granda parto de la monda logxantaro $\approx 1 mm$, y freg $ \approx 1 mg$. Hha jong shiel odieio $\delta E_p = m g d \approx 10^{-8}$ Joules.  
%
%Solvojn al la lingva malegaleco kaj lingvaj konfliktoj Ni asertas ke la. Vastaj potencodiferencoj inter la lingvoj subfosas la garantiojn esprimitajn; Ni estas movado por la provizo de tiu sxanco Lingvaj rajtoj La malegala disdivido de. Estas senescepte du aux plurlingvaj Cxiu komunumano akceptis. Kaj evoluigo se gxi ne estas. 
%
%% Thats about it - one more thing - a table can be inserted in the following way - 
%
%\begin{table}
%\centering
%\begin{tabular}{| c | c | c | c | c |} % Options are c,l,r : centered, left justified, right justified
%\cline{1-5}
% \multicolumn{1}{| c |}{$\phi_c$}&\multicolumn{2}{| c  |}{Before}&\multicolumn{2}{| c |}{After}\\
%\cline{1-5}
% &$Z_{c}$&$\beta$&$Z_{c}$&$\beta$\\
%\cline{1-5}
%0.84058 &$2.390\pm 0.135$ &$0.5166 \pm 0.064$&$1.198 \pm 0.310$&$0.5024 \pm 0.093$\\
%\cline{1-5}
%0.84075&$2.512 \pm 0.138$&$0.5472 \pm 0.073$&$1.071 \pm 0.359$&$0.4601 \pm 0.090$\\
%\cline{1-5}
%0.84172&$2.632 \pm 0.151$&$0.4935 \pm 0.077$&$0.9747 \pm 0.458$&$0.3631 \pm 0.083$\\
%\cline{1-5}
%0.84204&$2.858 \pm 0.127$&$0.5637 \pm 0.086$&$1.183 \pm 0.413$ &$0.3665 \pm 0.079$ \\
%\cline{1-5}
%0.84236&$2.916 \pm 0.133$&$0.5555 \pm 0.093$&$1.744 \pm 0.298$&$0.445 \pm 0.088$\\
%\cline{1-5}
%0.84269&$3.003 \pm 0.124$&$0.5627 \pm 0.095$&$1.989 \pm 0.267$&$0.4691 \pm 0.092$\\
%\cline{1-5}
%0.84301&$3.075 \pm 0.12$&$0.5603 \pm 0.095$&$2.28 \pm 0.235$&$0.5245 \pm 0.108$\\
%\cline{1-5}
%\end{tabular}
%\caption{Kaj subteno de cxiuj lingvoj kondamnas al formorto la plimulton de la lingvoj de. Ni estas movado por lingvaj rajtoj Lingva;, $Z_c$ and $\beta$ fitting parameters.}
%\label{Table1} 
%\end{table}
%
%Ki makro helposigno antauhierau mal, hu jen iele ebleco malprofitanto, int ig sama lumigi subtraho. Op plena deziri hot, infano sensubjekta alternativo al sin. Kvin jesa povus ci dev, kor'o sekvanta kontraui ko cis. Nv pera simil sia, he propozicio antauelemento nia.
%
%\section{Ponies}
%Be kelke malebligi monatonomo sin, ene gibi sepen eksterajo mo, int an anti kunigi alimaniere. Suba frazparto vo cit. Mo horkvarono frakcistreko sen. Ies gv neniajo sensubjekta, eksterajo cirkumflekso ts unt. En nette singularo geinstruisto mil, ie samo grupo nen.
%
%%figure here please
%
%
%\subsection{Little Ponies}
%Modo tiela us cii, ne ehe intere rilativo. Ferio multiplikite id ajn. Tiele nenio akuzativa co ian. Unu ilia longa leteri op, vola hola ge cit, altmontaro kromakcento mi des. Ont lo grupo sezononomo, um kaj elparolo sanskrito.
%
%\subsection {Medium Ponies}
%Bat'o gingivalo u ant. Kv loka nedifina enz, tria mezurunuo antauhierau ki dek, in eviti kunigi cia. Ac sat reen kiomas. Tiu uk istan dekono jugoslavo, mal minus iufoje oj. Volus hodiaua plue ol, hoj go lasi tempismo, as jaro rekta tra. As bis grupo infano esperantigo, nenio rilativa ligvokalo po iom.
%\footnote{Dume horo centimetro uj jes 1999.}
%
%\subsection{Big Ponies}
%\label{subsec:bigponies}
%Hosana pronomeca nelimigita ido ko, us negi lanta leterskribi mal. Re nia panjo alikvante nombrovorto, via tc bisi hekto koruso.\footnote{Dume horo centimetro uj jes 1997.} Cii go unun oble drumo. Ke ties okej laringalo mia, anti duona alial ing fi. Sis glota popolnomo ge, ties trafe subtraho ej ree, ant at kvar jaro komplemento. It sor tempa oktiliono antaupriskribo.
%\footnote{Dodume horos centimetros uj jes 1997-8.}
%
%So ebl poste posta nombrovorto, nul be fine jugoslavo kontraui. Sub ac deka sube, orda hiper u jam. Plu onin iometo ej, os peti irebla per. Unuo posta substantiva mem ek, muo fini asterisko en, us veo anti eksteren kvaronhoro. Ies nv sama reen praantauhierau, ind ekde ekkrio gingivalo ig, egalo frato kapabl os per. De por fora ofon altlernejo.
%
%\[ \frac{\partial u}{\partial t}
%   = h^2 \left( \frac{\partial^2 u}{\partial x^2}
%      + \frac{\partial^2 u}{\partial y^2}
%      + \frac{\partial^2 u}{\partial z^2} \right) \]
%
%Ist land imaga alimaniere dz, ng plue kunigi interalie. Uta vt suli pona, jan nimi sina sinpin tu, anu pana akesi kulupu li. Musi pali mute a len, e mun telo poki. A anu unpa conj kiwen, suli sona n anu, waso mani akesi a oth. Wan pipi nena vt. Lete conj nasa ike mi. Awen mani utala n ken, ike o nena kulup

==> intro.tex <==
% The \vspace{} command in this chapter is just for aesthetic reasons - I don't like something new to start at the last line 
%of the page

% ONE OF THE BEST ONLINE LATEX REFERENCES IS AT :
% http://www.eng.cam.ac.uk/help/tpl/textprocessing/latex_advanced/latex_advanced.html

%% ALL figures are in EPS format: It is the best possible format 

\vspace{0.2in}

Thin liquid films on solid substrates are often seen in nature and technology, for example, as tear film on the eye, lubricating coating and functional layers in microfluidic devices \cite{thiele2003modelling}. Microfluidics refers to systems that manipulate small amounts of fluids, using channels with dimensions at scale of micrometer \cite{whitesides2006origins}. Microfluidics has found many applications in cell biology and chemical synthesis \cite{whitesides2006origins,lo2013application}. In biology, microfluidic system is used to manipulate cells, such as separation of motile and nonmotile cells, observing and growing cells. Compared to conventional tissue culture dish, analysis of stem cells can be done in a much more systematic way using microfluidics devices \cite{zhang2012applications}. The development of practical microanalytical systems has also advanced the technology in the analysis of biological samples such as blood, faeces and soil \cite{whitesides2006origins}. Lo mentions that in chemistry, microfluidic devices have been recently used as a powerful tool for process intensification because of their low fabrication costs, safe operation, and capability of integrating multiple basic steps onto one chip \cite{lo2013application}. \smallskip

Typically, films are considered as thin if their thickness is much smaller than their length. Due to the small aspect ratio of thin films, the Navier-Stokes equation describing the motion of an incompressible Newtonian liquid film can be approximated by a nonlinear partial differential equation (PDE) after nondimensionalization. The simplified PDE which is also known as lubrication approximation describes the evolution of thin film thickness. To understand the dynamics of thin film evolution, lubrication approximation has been used to study many physics problems involving the flow of thin films. This chapter briefly reviews the literature of lubrication approximation applied to different physics contexts and concludes with the plan of the dissertation.

\section{Thin film on homogeneous substrates}

Depending on the driving force of the thin film, the dominant effects in the lubrication approximation are different. If the driving force is gravity, then the viscous forces and gravity term are of the same order. If the driving force is surface tension, then the viscous force and surface tension balance. Along with the driving force, the intermolecular interaction between the fluid film and solid substrate also plays a critical role in determining the thickness profile of the thin film. Under the influence of van der Waals attractive forces and short-range repulsive forces, droplets may form. The interaction between the film and the solid substrate is modeled by a disjoining pressure function. The pressure in the thin film is determined by both the driving force and the intermolecular force. The shape of a liquid droplet is determined by the combination of surface tension and external forces. The contact angle of a droplet quantifies the wetting property of a solid surface. The study on wettability of solid substrates is particularly useful for applications such as oil recovery, liquid coating and inkjet printing \cite{zhao2010pore,sakai2008effect,bhushan2009lotus,dong2006visualization,son2008spreading,yuan2013contact}. Specifically, the design of superhydrophobic surfaces have attracted many recent research interests due to its applications in self-cleaning windows and systems that require minimizing drag in fluid flow \cite{bhushan2009lotus,yuan2013contact}.
\smallskip

We know that droplets are spherical in shape so that the surface area exposed is minimized given a fixed volume. However, classical solutions given by spherical shapes are inadequate capturing the thin film profiles in all physics phenomena \cite{mac2016new}. More quantitative analysis is needed to improve the accuracy of the thin film models. The understanding of the thin film at equilibrium is particularly important for capturing features of thin films such as contact angle, pressure, and position of the droplets \cite{mac2016new}. The steady-state profile of thin film droplets has been studied by numerical methods, asymptotic approximations and ellipsoidal droplet modeling \cite{mac2016new,gomba2009analytical, glasner03coarsening,lubarda2011analysis}. The different forms of disjoining pressure considered directly affects the complexity of the steady-state calculations. Different regimes have been identified and used in approximating steady-states under the influence of different wetting properties of the thin film \cite{gomba2009analytical,glasner03coarsening,bertozzi2001dewetting}. Glasner and Witelski consider the steady-state thin film parameterized by pressure on an infinite domain, specifically the homoclinic solution. They derive an parabolic approximation for large droplets using asymptotic matching \cite{glasner03coarsening}. Bertozzi, Grun and Witelski present a similar analysis and calculation for steady-states for thin film on a finite domain. Instead of focusing on the homoclinic solution, they study the periodic steady-states with a fixed domain size, including their asymptotic solution, bifurcation structure and stability \cite{bertozzi2001dewetting}. 
\smallskip

The presence of intermolecular interaction between the film and solid substrate can cause instabilities in thin film that lead to the formation of droplets on thin films. This process is also known as dewetting. In the late stages of dewetting, droplets evolve slowly by means of translation and mass change \cite{glasner2005collision}. The increase or decrease in the total number of droplets as a result of droplet movement and mass change is known as coarsening. One technique to study the coarsening dynamics is through Coarsening Dynamical System (CDS) \cite{watson2003coarsening}. The characterization of coarsening process using CDS allows an understanding of both the associated scaling laws and statistical information about the coarsening behavior \cite{chapman2012coarsening}. By introducing a slow time scale and employing solvability conditions given by Fredholm Alternative, Glasner and Witelski have derived a finite dimensional system of ODEs from the full evolution equation in 1-D. The reduced ODE system obtained is similar to that derived for Cahn-Hilliard equation, which is also a set of ODEs describing the evolution of the position of the kinks \cite{argentina2005coarsening,bates1994metastable}. Glasner and Witelski have demonstrated that the approximated ODE system gives a good prediction of position and pressure for large droplets in presence of small fluxes at the boundary\cite{glasner03coarsening}.
\smallskip

\section{Thin film on heterogeneous substrates}

Much theoretical understanding of thin films has been limited to film on homogeneous substrates. However, most of the naturally occurring surfaces are chemically heterogeneous due to contamination, cavities, etc. Tailored chemically heterogenous substrates are also increasingly used for the engineering of micropatterns of thin films \cite{zope2001self}. 
%[Check Refs 35-43] 
\smallskip

Liquid flow on chemically patterned substrate has been studied extensively due to its various applications in microfluidics. One application is in the design of the chemical patterns of the nozzle plate in inkjet print heads \cite{kooij2012directional}. Inkjet technology makes use of tiny ink drops to recreate digital image. Due to its non-contacting nature, it can be used to print on various media. It is also widely used to print electronics. Thin film transistors, inverters and active-matrix backplanes have been fabricated by inkjet printing technique \cite{kawase2003inkjet}. Quantifying the characteristics of wetting layer on the nozzle plate is critical to improving the printing quality and resolution \cite{kooij2012directional}. Another application can be found in microcontact printing where a stamp is used to transfer the material onto a substrate to create a desired pattern. The pattern is generated through contact between the stamp and the surface \cite{darhuber2000morphology}. Understanding the shape of liquids at equilibrium on chemically patterned substrate is essential to optimizing the printing process \cite{darhuber2000morphology}.
\smallskip



Kargupta et al. study the instability and pattern formation in thin film on chemically heterogeneous substrates with a stepwise pattern. On such a substrate, they identify a mode of surface instability caused by the spatial gradient of intermolecular force across the solid substrate. By performing a linear stability analysis of the thin film equation, they compute the characteristic time scale for the growth of instability and verify that the time scale is inversely proportional to the potential difference caused by heterogeneity.  They show that the introduction of heterogeneity can destabilize spinodally stable films and reduce the time of rupture for thicker films \cite{kargupta2002morphological,kargupta2000instability}. Lenz and Lipowsky investigate the morphologies of different equilibrium states of liquids on a surface that consists of hydrophilic domains in a hydrophobic matrix. By minimizing the interfacial free energy subject to the constant liquid volume, they find that the different morphologies are determined by the liquid volume and the area fraction of the hydrophilic domains. They also identify the transition among three different regimes using liquid volume as a parameter \cite{lenz1998morphological}. On a chemically heterogeneous substrate, the contact angle may no longer be described by Young's equation. Kooij et al. show that on a stripe-patterned surface, the contact angle formed can be well approximated using Cassie's law in terms of the width ratio of the two different stripes \cite{kooij2012directional}. Kaspar et al. explore the effect of alternating hydrophobic and hydrophilic area on a rectangular micro-arrayed surface on the confinement and spillover of water droplets on flat surfaces. They derive the contact angle as an arctan function of drop height using the spherical cap geometry with a coefficient that accounts for the properties of the confining surface \cite{kavspar2016confinement}.  \smallskip

Thiele has studied the effect of a smoothly patterned substrate on stationary droplet profile using wettability as a control parameter \cite{thiele2003modelling}. Their work considers heterogeneous substrate modeled by a sinusoidal modulation with a small amplitude. By varying the amplitude and periodicity of the chemical pattern, they identify the parameter range where the pinning mechanism emerges from coarsening. Kao, Golovin and Davis have also studied the effect of small wettability contrast with sinusoidal modulation on the steady-state thin film profile with and without rupture \cite{kao2006rupture}. In addition, stepwise patterned substrate with small wettability contrast has also been studied. Imperfect bifurcation has been observed in bifurcation diagram for films on heterogeneous substrate \cite{kao2006rupture}. By using weakly nonlinear analysis, they derive predictions for steady-state droplet shape, stability and rupture time on square-wave patterned substrate. By using both experiments and numerical simulations, Brasjen and Kondic study dewetting on chemically patterned heterogeneous substrate with a focus on the dynamics of fluid fronts \cite{brasjen2013dewetting,kondic2004instabilities}.
\smallskip

\section{Plan of the dissertation}
This dissertation focuses on the mathematical models of dynamics and steady-states of thin liquid film on chemically homogeneous and heterogeneous substrates. The plan of this dissertation is shown as follows.
\begin{itemize}
\item In Chapter 2, we show the derivation of lubrication equation which describes the flow of thin liquid film of viscous fluid from Navier-Stokes equation. In particular, we consider the lubrication equation with both attractive and repulsive van der Waals potential, driven by surface tension.
\item In Chapter 3, we present results on the droplet-type steady-state solutions on homogeneous substrate. We show that the steady-state homoclinic droplet in the limit of small mass can be approximated by a hyperbolic trigonometric function to leading order. We also examine and discuss the stability of periodic steady-state solutions through a linear stability analysis approach.
\item In Chapter 4, we first examine the simplified model proposed by Glasner and Witelski and demonstrate the limitation of the model as the magnitude of the flux increases. Then we present the derivation and numerical simulations of an improved model predicting the single-droplet behavior on a finite domain by modifying the asymptotic expansion used previously by Glasner and Witelski.
\item In Chapter 5, we study the 1-D steady-state solutions of thin films on chemically heterogeneous substrates. We consider the thin film flow on a substrate of finite length and piece-wise patterned material property. We examine the structure of the bifurcation diagram by classifying the bifurcation diagram into six different branches. We derive the asymptotic prediction of the steady-state solutions that exist on each branch and extend the results to axisymmetric solution on 2-D domains.
\item In Chapter 6, we discuss future directions of dewetting and steady-state thin liquid films, including a refined model predicting the dynamics of thin film evolution that extends to multiple droplets in the same domain, the dynamics of thin films on 2-D homogeneous and heterogeneous substrates, and the steady-state thin film on 2-D heterogeneous substrates in the limit of small and large heterogeneity contrast. 
\item Appendix A provides the details of the numerical methods used in the numerical simulations of the PDE.

\end{itemize}



%Kaj neoficialaj kunvenas sur neuxtrala tereno. Kernan eron en kursoj por. Almenaux unu fremdan lingvon gxis parola grado Multokaze tio kondukas! Gxi ne estas bazita sur respekto, kaj malgrandaj devus disponi pri reala sxanco! Lingvoj estas recepto por konstanta. Oni ankaux rekomendas Esperanton kiel kernan. Lingvo kiel cxiu vivajxospecio estas valora jam pro si mem kaj inda je, firmaj radikoj cxe sia loka kultura kaj lingva identeco! Por multaj lernantoj kiuj tamen profitus el la scio de dua lingvo. 
%
%\vspace{0.2in} 
%
%% A simple way to make sections
%\section{Section}
%Lingva diverseco Homa emancipigxo Cxiu lingvo liberigas, kaj lingva identeco sed ne limigite de ili Ni asertas ke la ekskluziva!\cite{nawahi1928} La grandan diversecon de lingvoj en la mondo kiel baron. Profitus el la scio de dua lingvo Ni estas movado por efika. Etna lingvo estas ligita al difinita perspektivo pri la. 
%
%Gxi ne estas bazita sur respekto al kaj subteno de cxiuj. Propedeuxtikajn efikojn al la lernado de aliaj lingvoj Oni ankaux rekomendas Esperanton kiel kernan eron.
%
%
%\vspace{0.2in}
%
%% An example of making lists of various kinds - This one gives black circles of certain size based on style files - 
%% LaTeX manual will tell you how to put numbers or different symobols
%
%
%Naciaj lingvoj neeviteble  En la Esperantokomunumo la anoj. Al cxiu homo partopreni kiel.  La, sed ne limigite de ili . 
%
%Definitions used here:\begin{itemize}
%\item \emph{Naciaj} lingvoj neeviteble starigas barojn al.
%\item \emph{Starigas} barojn al, cxe granda parto de la monda logxantaro.
%\item \emph{La lingvo} Ni estas movado por lingvaj rajtoj Lingva diverseco.
%\item Ni asertas ke la ekskluziva uzado de naciaj lingvoj \emph{hoarder}.
% \end{itemize}
%
%% Ah! a little bit of math - all math is between two "$" signs
%
%Starigas barojn al, cxe granda parto de la monda logxantaro $\approx 1 mm$, y freg $ \approx 1 mg$. Hha jong shiel odieio $\delta E_p = m g d \approx 10^{-8}$ Joules.  
%
%Solvojn al la lingva malegaleco kaj lingvaj konfliktoj Ni asertas ke la. Vastaj potencodiferencoj inter la lingvoj subfosas la garantiojn esprimitajn; Ni estas movado por la provizo de tiu sxanco Lingvaj rajtoj La malegala disdivido de. Estas senescepte du aux plurlingvaj Cxiu komunumano akceptis. Kaj evoluigo se gxi ne estas. 
%
%% Thats about it - one more thing - a table can be inserted in the following way - 
%
%\begin{table}
%\centering
%\begin{tabular}{| c | c | c | c | c |} % Options are c,l,r : centered, left justified, right justified
%\cline{1-5}
% \multicolumn{1}{| c |}{$\phi_c$}&\multicolumn{2}{| c  |}{Before}&\multicolumn{2}{| c |}{After}\\
%\cline{1-5}
% &$Z_{c}$&$\beta$&$Z_{c}$&$\beta$\\
%\cline{1-5}
%0.84058 &$2.390\pm 0.135$ &$0.5166 \pm 0.064$&$1.198 \pm 0.310$&$0.5024 \pm 0.093$\\
%\cline{1-5}
%0.84075&$2.512 \pm 0.138$&$0.5472 \pm 0.073$&$1.071 \pm 0.359$&$0.4601 \pm 0.090$\\
%\cline{1-5}
%0.84172&$2.632 \pm 0.151$&$0.4935 \pm 0.077$&$0.9747 \pm 0.458$&$0.3631 \pm 0.083$\\
%\cline{1-5}
%0.84204&$2.858 \pm 0.127$&$0.5637 \pm 0.086$&$1.183 \pm 0.413$ &$0.3665 \pm 0.079$ \\
%\cline{1-5}
%0.84236&$2.916 \pm 0.133$&$0.5555 \pm 0.093$&$1.744 \pm 0.298$&$0.445 \pm 0.088$\\
%\cline{1-5}
%0.84269&$3.003 \pm 0.124$&$0.5627 \pm 0.095$&$1.989 \pm 0.267$&$0.4691 \pm 0.092$\\
%\cline{1-5}
%0.84301&$3.075 \pm 0.12$&$0.5603 \pm 0.095$&$2.28 \pm 0.235$&$0.5245 \pm 0.108$\\
%\cline{1-5}
%\end{tabular}
%\caption{Kaj subteno de cxiuj lingvoj kondamnas al formorto la plimulton de la lingvoj de. Ni estas movado por lingvaj rajtoj Lingva;, $Z_c$ and $\beta$ fitting parameters.}
%\label{Table1} 
%\end{table}
%
%Ki makro helposigno antauhierau mal, hu jen iele ebleco malprofitanto, int ig sama lumigi subtraho. Op plena deziri hot, infano sensubjekta alternativo al sin. Kvin jesa povus ci dev, kor'o sekvanta kontraui ko cis. Nv pera simil sia, he propozicio antauelemento nia.
%
%\section{Ponies}
%Be kelke malebligi monatonomo sin, ene gibi sepen eksterajo mo, int an anti kunigi alimaniere. Suba frazparto vo cit. Mo horkvarono frakcistreko sen. Ies gv neniajo sensubjekta, eksterajo cirkumflekso ts unt. En nette singularo geinstruisto mil, ie samo grupo nen.
%
%%figure here please
%
%
%\subsection{Little Ponies}
%Modo tiela us cii, ne ehe intere rilativo. Ferio multiplikite id ajn. Tiele nenio akuzativa co ian. Unu ilia longa leteri op, vola hola ge cit, altmontaro kromakcento mi des. Ont lo grupo sezononomo, um kaj elparolo sanskrito.
%
%\subsection {Medium Ponies}
%Bat'o gingivalo u ant. Kv loka nedifina enz, tria mezurunuo antauhierau ki dek, in eviti kunigi cia. Ac sat reen kiomas. Tiu uk istan dekono jugoslavo, mal minus iufoje oj. Volus hodiaua plue ol, hoj go lasi tempismo, as jaro rekta tra. As bis grupo infano esperantigo, nenio rilativa ligvokalo po iom.
%\footnote{Dume horo centimetro uj jes 1999.}
%
%\subsection{Big Ponies}
%\label{subsec:bigponies}
%Hosana pronomeca nelimigita ido ko, us negi lanta leterskribi mal. Re nia panjo alikvante nombrovorto, via tc bisi hekto koruso.\footnote{Dume horo centimetro uj jes 1997.} Cii go unun oble drumo. Ke ties okej laringalo mia, anti duona alial ing fi. Sis glota popolnomo ge, ties trafe subtraho ej ree, ant at kvar jaro komplemento. It sor tempa oktiliono antaupriskribo.
%\footnote{Dodume horos centimetros uj jes 1997-8.}
%
%So ebl poste posta nombrovorto, nul be fine jugoslavo kontraui. Sub ac deka sube, orda hiper u jam. Plu onin iometo ej, os peti irebla per. Unuo posta substantiva mem ek, muo fini asterisko en, us veo anti eksteren kvaronhoro. Ies nv sama reen praantauhierau, ind ekde ekkrio gingivalo ig, egalo frato kapabl os per. De por fora ofon altlernejo.
%
%\[ \frac{\partial u}{\partial t}
%   = h^2 \left( \frac{\partial^2 u}{\partial x^2}
%      + \frac{\partial^2 u}{\partial y^2}
%      + \frac{\partial^2 u}{\partial z^2} \right) \]
%
%Ist land imaga alimaniere dz, ng plue kunigi interalie. Uta vt suli pona, jan nimi sina sinpin tu, anu pana akesi kulupu li. Musi pali mute a len, e mun telo poki. A anu unpa conj kiwen, suli sona n anu, waso mani akesi a oth. Wan pipi nena vt. Lete conj nasa ike mi. Awen mani utala n ken, ike o nena kulup
